Visual Prompt Tuning for Generative Transfer Learning

Transferring knowledge from an image synthesis model trained on a large dataset is a promising direction for learning generative image models from various domains efficiently. While previous works have studied GAN models, we present a recipe for learning vision transformers by generative knowledge transfer. We base our framework on state-of-the-art generative vision transformers that represent an image as a sequence of visual tokens to the autoregressive or non-autoregressive transformers. To adapt to a new domain, we employ prompt tuning, which prepends learnable tokens called prompt to the image token sequence, and introduce a new prompt design for our task. We study on a variety of visual domains, including visual task adaptation benchmark~\cite{zhai2019large}, with varying amount of training images, and show effectiveness of knowledge transfer and a significantly better image generation quality over existing works.

==> setup/math.tex <==
\usepackage{amsmath,amsfonts,bm}

\def\argmax{\mathop{\rm argmax}}%
\def\argmin{\mathop{\rm argmin}}%


\def\bx{\bm{x}} %
\def\bxp{\bm{x}^{\prime}} %
\def\bxpp{\bm{x}^{\prime\prime}} %
\def\tbx{\tilde{\bm{x}}} %
\def\hbx{\hat{\bm{x}}} %
\def\ex{e(\bm{x})}
\def\tex{e({\tilde{\bm{x}}})}

\def\by{\bm{y}} %
\def\byp{\bm{y}^{\prime}} %
\def\bypp{\bm{y}^{\prime\prime}} %
\def\tby{\tilde{\bm{y}}} %
\def\ty{\tilde{{y}}} %
\def\hby{\hat{\bm{y}}} %
\def\ey{e(\bm{y})}
\def\tey{e({\tilde{\bm{y}}})}

\def\vw{\bm{w}}


\def\anchor{\overline{D}}

\def\reg{R_{\mathrm{LC}}}


\def\bv{\bm{v}} %
\def\tv{\tilde{v}} %
\def\tbv{\tilde{\bm{v}}} %

\usepackage{amsmath,amsfonts}
\usepackage{bbm}

\newcommand{\eat}[1]{} % ignores argument


%GAN
\def\pd{p_d(\bx)} %
\def\pg{p_g(\bx)} %
\def\pz{p_z(\bx)} %
\def\Dx{D(\bx)} %
\def\Dsx{D^*(\bx)} %



\def\N{\mathcal{N}} %
\def\Z{\mathcal{Z}} %
\def\E{\mathop{\mathbb{E}}} %
